Learning to Locate: GNN-Powered Vulnerability Path Discovery in Open Source Code

Detecting security vulnerabilities in open-source software is a critical task that is highly regarded in the related research communities. Several approaches have been proposed in the literature for detecting vulnerable codes and identifying the classes of vulnerabilities. However, there is still room to work in explaining the root causes of detected vulnerabilities through locating vulnerable statements and the discovery of paths leading to the activation of the vulnerability. While frameworks like SliceLocator offer explanations by identifying vulnerable paths, they rely on rule-based sink identification that limits their generalization. In this paper, we introduce VulPathFinder, an explainable vulnerability path discovery framework that enhances SliceLocator's methodology by utilizing a novel Graph Neural Network (GNN) model for detecting sink statements, rather than relying on predefined rules. The proposed GNN captures semantic and syntactic dependencies to find potential sink points (PSPs), which are candidate statements where vulnerable paths end. After detecting PSPs, program slicing can be used to extract potentially vulnerable paths, which are then ranked by feeding them back into the target graph-based detector. Ultimately, the most probable path is returned, explaining the root cause of the detected vulnerability. We demonstrated the effectiveness of the proposed approach by performing evaluations on a benchmark of the buffer overflow CWEs from the SARD dataset, providing explanations for the corresponding detected vulnerabilities. The results show that VulPathFinder outperforms both original SliceLocator and GNNExplainer (as a general GNN explainability tool) in discovery of vulnerability paths to identified PSPs.

==> Theorem-Styles.tex <==
\RequirePackage{amsthm}%
\def\th@plain{%
\thm@preskip\parskip
\thm@postskip\z@
\itshape % body font
}
\def\th@definition{%
\thm@preskip\parskip
\thm@postskip\z@
\normalfont % body font
}
\def\th@remark{%
\thm@headfont{\itshape}%
\normalfont % body font
\thm@preskip\parskip \divide\thm@preskip\tw@
\thm@postskip\z@
}

%\newenvironment{pf}%
%  {\par\addvspace{\@bls \@plus 0.5\@bls \@minus 0.1\@bls}\noindent
%   {\bfseries\Elproofname}\enspace\ignorespaces}%
%  {\par\addvspace{\@bls \@plus 0.5\@bls \@minus 0.1\@bls}}
%\def\Elproofname{PROOF.}
%\@namedef{pf*}#1{\par\begingroup\def\Elproofname{#1}\pf\endgroup\ignorespaces}
%\expandafter\let\csname endpf*\endcsname=\endpf


\newtheoremstyle{XYZ}% name
{3pt}% Space above
{3pt}% Space below
{}% Body font
{}% Indent amount
{\bfseries}% Theorem head font
{}% Punctuation after theorem head
{.5em}% Space after theorem head
{\bfseries{#1 #2\if#3\else~(#3)\fi.}}% Theorem head spec (can be left empty, meaning `normal')



\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
\newtheorem{axiom}{Axiom}
\newtheorem{conjecture}{Conjecture}
\newtheorem{fact}{Fact}
\newtheorem{hypothesis}{Hypothesis}
\newtheorem{assumtion}{Assumption}
\newtheorem{criterion}{Criterion}
\theoremstyle{XYZ}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{notation}{Notation}
\newtheorem{problem}{Problem}
\newtheorem{principle}{Principle} 
